Denotational Semantics and a Fast Interpreter for jq

jq is a widely used tool that provides a programming language to manipulate JSON data. However, its semantics are currently only specified by its implementation, making it difficult to reason about its behaviour. To this end, I provide a syntax and denotational semantics for a subset of the jq language. In particular, the semantics provide a new way to interpret updates. I implement an extended version of the semantics in a novel interpreter for the jq language called jaq. Although jaq uses a significantly simpler approach to execute jq programs than jq, jaq is faster than jq on ten out of thirteen benchmarks.

==> tikz/bind-many.tex <==
\begin{tikzpicture}
\coordinate (source);

\node (f)  [minimum size=30,right=0.5 of source,draw] {$f$};
\coordinate (fo1) at ($ (f.north east) !.25! (f.east) $);
\coordinate (fo2) at ($ (f.south east) !.25! (f.east) $);

\node (g1) [minimum size=16,above right=0.5 and 1 of fo1,draw] {$g$};
\node (g2) [minimum size=16,below right=0.5 and 1 of fo2,draw] {$g$};

\draw (source) -- +(-1,0);
\draw [->,clone] (source) -- (f);
\draw [->,clone] (source) |- (g1);
\draw [->,clone] (source) |- (g2);

\draw [->] (fo1) -| node[near end,left] {$\$x$} (g1);
\draw [->] (fo2) -| node[near end,left] {$\$x$} (g2);

\node [right=0.3 of f ] {$\rvdots$};
\node at ($(g1.center) !.5! (g2.center) $) {$\rvdots$};
\node [right=0.3 of g1] {$\rvdots$};
\node [right=0.3 of g2] {$\rvdots$};

\draw [->] ($ (g1.north east) !.25! (g1.east) $) -- +(1,0);
\draw [->] ($ (g1.south east) !.25! (g1.east) $) -- +(1,0);
\draw [->] ($ (g2.north east) !.25! (g2.east) $) -- +(1,0);
\draw [->] ($ (g2.south east) !.25! (g2.east) $) -- +(1,0);

\node [filter,fit=(source) (g1) (g2),label={$f \as \$x \mid g$}] {};
\end{tikzpicture}


==> tikz/bind-single.tex <==
\begin{tikzpicture}
\coordinate (source);

\node (f) [minimum size=30,right=0.5 of source,draw] {$f$};
\node (g) [minimum size=16,above right=0.5 and 1 of f.east,draw] {$g$};

\draw (source) -- +(-1,0);
\draw [->,clone] (source) -- (f);

\draw [->] (f) -| node[near end,left] {$\$x$} (g);
\draw [->] (source) |- (g);

\node [right=0.3 of g] {$\rvdots$};

\draw [->] ($ (g.north east) !.25! (g.east) $) -- +(1,0);
\draw [->] ($ (g.south east) !.25! (g.east) $) -- +(1,0);

\node [filter,fit=(source) (f) (g),label={$f \as \$x \mid g$}] {};
\end{tikzpicture}


==> tikz/compose.tex <==
\begin{tikzpicture}
\coordinate (source);

\node (f)  [minimum size=40,right=of source,draw] {$f$};
\coordinate (fo1) at ($ (f.north east) !.25! (f.east) $);
\coordinate (fo2) at ($ (f.south east) !.25! (f.east) $);

\node (g1) [minimum size=16,right=of fo1,draw] {$g$};
\node (g2) [minimum size=16,right=of fo2,draw] {$g$};

\draw [->] (source) -- (f);
\draw [->] (fo1) -- (g1);
\draw [->] (fo2) -- (g2);

\node [right=0.3 of f ] {$\rvdots$};
\node at ($(g1.center) !.5! (g2.center) $) {$\rvdots$};
\node [right=0.3 of g1] {$\rvdots$};
\node [right=0.3 of g2] {$\rvdots$};

\draw [->] ($ (g1.north east) !.25! (g1.east) $) -- +(1,0);
\draw [->] ($ (g1.south east) !.25! (g1.east) $) -- +(1,0);
\draw [->] ($ (g2.north east) !.25! (g2.east) $) -- +(1,0);
\draw [->] ($ (g2.south east) !.25! (g2.east) $) -- +(1,0);

\node [filter,fit=(f) (g1) (g2),label={$f \mid g$}] {};
\end{tikzpicture}


==> tikz/concat.tex <==
\begin{tikzpicture}
\coordinate (source);
\node (f) [minimum size=20,above right=0.1 and 0.5 of source,draw] {$f$};
\node (g) [minimum size=20,below right=0.1 and 0.5 of source,draw] {$g$};

\draw (source) -- +(-1,0);
\draw [->,clone] (source) |- (f);
\draw [->]       (source) |- (g);

\node [right=0.3 of f] {$\rvdots$};
\node [right=0.3 of g] {$\rvdots$};

\draw [->] ($ (f.north east) !.25! (f.east) $) -- +(1,0);
\draw [->] ($ (f.south east) !.25! (f.east) $) -- +(1,0);
\draw [->] ($ (g.north east) !.25! (g.east) $) -- +(1,0);
\draw [->] ($ (g.south east) !.25! (g.east) $) -- +(1,0);

\node [filter,fit=(source) (f) (g),label={$f, g$}] {};
\end{tikzpicture}


==> tikz/eval.tex <==
\begin{tikzpicture}
\begin{axis}[
  ybar=1pt,
  x=1cm,
  xtick=data,
  xtick style={draw=none},
  ymin=0,
  enlarge y limits={abs=5ex,upper},
  enlarge x limits={abs=0.5cm},
  symbolic x coords={
    empty,
    bf-fib,
    reverse,
    sort,
    add,
    kv,
    kv-update,
    kv-entries,
    ex-implode,
    reduce,
    tree-flatten,
    tree-update,
    to-fromjson,
  },
  xticklabels={
    empty-512,
    bf-fib-13,
    reverse-$2^{20}$,
    sort-$2^{20}$,
    add-$2^{20}$,
    kv-$2^{17}$,
    kv-update-$2^{17}$,
    kv-entries-$2^{17}$,
    ex-implode-$2^{20}$,
    reduce-$2^{20}$,
    tree-flatten-17,
    tree-update-17,
    to-fromjson-$2^{16}$,
  },
  ylabel=Runtime,
  y unit=s,
  nodes near coords,
  nodes near coords style={rotate=90,anchor=west,/pgf/number format/.cd,fixed zerofill,precision=2},
  x tick label style={rotate=45,anchor=east},
  ]

\addplot+ table [x=Filter, y expr=\thisrow{jq-time}] {tikz/eval.dat};
\addplot+ table [x=Filter, y expr=\thisrow{jaq-time}]{tikz/eval.dat};
\legend{jq, jaq}
\end{axis}

\end{tikzpicture}

